Neural Recording Power Optimization Through Machine Learning Guided Resolution Reconfiguration

Neural recording implants are a crucial tool for both neuroscience research and enabling new clinical applications. The power consumption of high channel count implants is dominated by the circuits used to amplify and digitize neural signals. Since circuit designers have pushed the efficiency of these circuits close to the theoretical physical limits, reducing power further requires system level optimization. Recent advances use a strategy called channel selection, in which less important channels are turned off to save power. We demonstrate resolution reconfiguration, in which the resolution of less important channels is scaled down to save power. Our approach leverages variable importance of each channel inside machine-learning-based decoders and we trial this methodology across three applications: seizure detection, gesture recognition, and force regression. With linear decoders, resolution reconfiguration saves 8.7x, 12.8x, and 23.0x power compared to a traditional recording array for each task respectively. It further saves 1.6x, 3.4x, and 5.2x power compared to channel selection. The results demonstrate the power benefits of resolution reconfigurable front-ends and their wide applicability to neural decoding problems.

==> table.tex <==
\begin{document}
\begin{tabular}{c cccc cccc cccc cccc}
\toprule
$\delta$ & \multicolumn{4}{c}{Seizure} & \multicolumn{4}{c}{Melbourne} & \multicolumn{4}{c}{Gesture} & \multicolumn{4}{c}{Grasp} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
 & Sel. & Scal. & Rat. & Comp. & Sel. & Scal. & Rat. & Comp. & Sel. & Scal. & Rat. & Comp. & Sel. & Scal. & Rat. & Comp. \\
\midrule
\multicolumn{17}{l}{\textit{Absolute degradation}} \\
0.01 & 3.60 & 6.64 & 1.84 & 3.23 & 2.95 & 2.60 & 0.88 & 1.37 & 2.18 & 12.76 & 5.85 & 8.43 & 3.65 & 2.73 & 0.75 & 0.78 \\
0.02 & 4.07 & 7.55 & 1.86 & 3.45 & 4.09 & 3.56 & 0.87 & 1.35 & 2.62 & 12.76 & 4.87 & 8.43 & 3.93 & 7.16 & 1.82 & 1.92 \\
0.03 & 4.58 & 8.26 & 1.80 & 3.21 & 4.68 & 4.06 & 0.87 & 1.55 & 3.03 & 12.76 & 4.22 & 8.43 & 4.04 & 13.66 & 3.38 & 3.43 \\
0.05 & 5.39 & 8.74 & 1.62 & 3.38 & 5.15 & 4.06 & 0.79 & 1.55 & 3.71 & 12.76 & 3.44 & 8.43 & 4.40 & 23.00 & 5.23 & 5.61 \\
0.10 & 8.09 & 9.69 & 1.20 & 3.55 & 5.15 & 8.01 & 1.55 & 2.24 & 4.72 & 12.76 & 2.70 & 8.43 & 6.02 & 39.31 & 6.53 & 8.39 \\
\midrule
\multicolumn{17}{l}{\textit{Relative degradation}} \\
0.01 & 3.49 & 6.64 & 1.91 & 3.23 & 2.75 & 2.60 & 0.95 & 1.37 & 2.16 & 12.76 & 5.90 & 8.43 & 3.52 & 2.09 & 0.60 & 0.60 \\
0.02 & 3.86 & 6.94 & 1.80 & 3.24 & 3.24 & 2.60 & 0.80 & 1.37 & 2.59 & 12.76 & 4.94 & 8.43 & 3.60 & 2.73 & 0.76 & 0.78 \\
0.03 & 4.13 & 7.70 & 1.87 & 3.21 & 4.09 & 2.60 & 0.64 & 1.37 & 3.00 & 12.76 & 4.25 & 8.43 & 3.71 & 3.56 & 0.96 & 0.99 \\
0.05 & 5.19 & 8.54 & 1.65 & 3.43 & 4.68 & 4.06 & 0.87 & 1.55 & 3.71 & 12.76 & 3.44 & 8.43 & 3.90 & 5.54 & 1.42 & 1.48 \\
0.10 & 5.94 & 9.28 & 1.56 & 3.58 & 5.15 & 6.50 & 1.26 & 1.82 & 4.65 & 12.76 & 2.74 & 8.43 & 4.10 & 15.89 & 3.88 & 3.96 \\
\bottomrule
\end{tabular}
\end{document}

